Detecting Machine-Generated Long-Form Content with Latent-Space Variables

The increasing capability of large language models (LLMs) to generate fluent long-form texts is presenting new challenges in distinguishing machine-generated outputs from human-written ones, which is crucial for ensuring authenticity and trustworthiness of expressions. Existing zero-shot detectors primarily focus on token-level distributions, which are vulnerable to real-world domain shifts, including different prompting and decoding strategies, and adversarial attacks. We propose a more robust method that incorporates abstract elements, such as event transitions, as key deciding factors to detect machine versus human texts by training a latent-space model on sequences of events or topics derived from human-written texts. In three different domains, machine-generated texts, which are originally inseparable from human texts on the token level, can be better distinguished with our latent-space model, leading to a 31% improvement over strong baselines such as DetectGPT. Our analysis further reveals that, unlike humans, modern LLMs like GPT-4 generate event triggers and their transitions differently, an inherent disparity that helps our method to robustly detect machine-generated texts.

==> content/old-intro.tex <==

% Introduce why latent variables? Refering to figure 1b
% Towards a more robust detection method, this paper investigate two pivotal questions: \textit{\textbf{1)}} What are the fundamental differences between human- and machine- authored text? We posit that a crucial distinction lies in the \textit{planning phase} of human writing, which, although not directly observable in the final text, significantly influences the \textit{\textbf{intermediate}}, or compositional, process. Conversely, machine text generation typically involves mere auto-regression. \yufei{The first QA is good reasoning but needs rewrite. It make people wrongly feel as long we as ask machines do planning before auto-regression, it will be the same as humans. We actually investigated planning using simple chain and complex chain prompting, and showed that's not the case. Talk about model failing at discourse/hidden structures, and that even with an explicit planning stage, the models cannot mimic humans. } \yufei{btw, I think you brought up a really good point -- we should state somewhere in the intro that we find such discourse incoherence/discrepancy cannot be improved with plan-and-write (simple chain) or self-reflect based revision (complex chain)... the discrepancy in hidden structure is more nuanced} \textit{\textbf{2)}} How do current adversarial attacks deceive existing detectors? We find adversarial attacks \cite{} typically involve replacing original texts with lexically different yet semantically similar alternatives, thereby fooling detectors by altering text distributions at the observational space.

% Combining these insights, we observe that current models and detectors predominantly focus on the text (token) generation processes, yet they overlook the intricate relationships within the text that are not explicitly expressed. By uncovering a method to represent these latent processes that underlie writing, we are able to develop more robust detectors capable of distinguishing between machine-generated and human-authored texts.\yufei{This paragraph is redundant with the previous one, can combine. Should really motivate latent features and emphasize that model struggle with discourse-level structures (need to give examples on what is discourse features, too)}


%%leading to discourse-level incoherence or missing anchored goals \cite{wang2022language_stochastic}. %A possible reason might be that human keep a high-level understanding \cite{hayes1987writing_structure} of the whole article in mind when writing, which determines the underlying framework or organization that shapes and guides the content to maintain discourse coherence, even though it might not be explicitly stated. 

% Introduce our approach, refer to figure 1 (b)
% Some researchers \yufei{directly cite} have already notice that LLMs, despite generating fluent text, often fail to capture the nuanced, high-level structure of extended texts, leading to content that lacks coherent discourse structure or reads as if the model has no anchored goal. \yufei{the previous two sentences fit well into your revised Question 1.} 

%To mitigate the problems of poor structure of text generated by language models, some previos work proposed latent generative processes to explicitly model or evaluate long-form coherence structure by utilizing annotated section transitions \cite{deng2022model_criticism} or sentence embeddings \cite{wang2022language_stochastic}. Thus, we are inspired to adopt a latent variable approach for MGT detection task.

%With the advent of large language models (LLMs), various approaches to detect machine-generated text (MGT) were developed. However, their robustness remains unsatisfying under realistic scenarios. Our paper analyzes the key factors influencing existing detectors: decoding setting, prompt and attack.This study proposes a method to perform detection with latent variables, which leverages the inherent defectiveness of current LLMs in learning hidden structures of human writing (\textit{e.g.}, event choices, topic transitions). It first projects text into latent space and then builds a more robust classifier on latent representations.
